Enhancing Neural Subset Selection: Integrating Background Information into Set Representations

Learning neural subset selection tasks, such as compound selection in AI-aided drug discovery, have become increasingly pivotal across diverse applications. The existing methodologies in the field primarily concentrate on constructing models that capture the relationship between utility function values and subsets within their respective supersets. However, these approaches tend to overlook the valuable information contained within the superset when utilizing neural networks to model set functions. In this work, we address this oversight by adopting a probabilistic perspective. Our theoretical findings demonstrate that when the target value is conditioned on both the input set and subset, it is essential to incorporate an \textit{invariant sufficient statistic} of the superset into the subset of interest for effective learning. This ensures that the output value remains invariant to permutations of the subset and its corresponding superset, enabling identification of the specific superset from which the subset originated. Motivated by these insights, we propose a simple yet effective information aggregation module designed to merge the representations of subsets and supersets from a permutation invariance perspective. Comprehensive empirical evaluations across diverse tasks and datasets validate the enhanced efficacy of our approach over conventional methods, underscoring the practicality and potency of our proposed strategies in real-world contexts.

==> sections/draft.tex <==
\section{Prelinimaries}
In this paper, we mainly consider the set data. Let $V = \{x_1,x_2,\dots,x_n \}$ with $x_i \in \gX$ denotes the input set under permutation group $\Symn.$ While $Y\in \mathbb{R}$ being a predicted output based on input $V.$

A permutation invariant function $f: \gV \to \gY$ is invariant to all permutations of the elements of $V$, i.e, for any permutation $\pi:$
\begin{align}\nonumber
    f(V) = f(\pi \cdot V) = f(\{x_{\pi(1)},x_{\pi(2)},\dots,x_{\pi(n)} \}).
\end{align}
The functional permutation invariance is defined when the output $Y$ is a deterministic map of $V$. From a probabilistic perspective, we can model the relationship between input $X$ and output $V$ by directly parameterizing the conditional distribution $P(Y|V)$, or by generating samples from $P(Y|V)$. Therefore, we can define the conditional distribution of $Y$ given $V,$ which has invariance properties with respect to $\Symn.$ Throughout, we assume all random variables are assumed to take values in standard Borel spaces and all maps introduced are measurable. Finally, $\equdist$ denotes equality in distribution, and $\equas$ denotes almost sure equality. Here, we can define the permutation invariant conditional distribution as:
\begin{definition}
Let $\gV$ and $\gY$ be the input and output spaces. The conditional distribution $P(Y|V)$ of $Y$ given $V$ is said to be \textit{invariant} under a group $\grp$ if the distribution of $Y$ keeps unchanged under the action of $\grp$ on $X$, i.e.,
\begin{align}\nonumber
P(Y\mid X) = P(Y\mid g\cdot X) \quad \text{for all } g\in\grp \;.
\end{align}
\end{definition}
Actually, constructing invariant conditional distribution $P(Y|X)$ requires the marginal distribution $P(X)$ to be an invariant distribution under $\Symn$. This is satisfied in the applications of our interest. For set-type data, it was assumed that the order of the elements in a set is unimportant, i.e., the set data $X$ is marginal invariant under the permutation group. More formally, we define it as follows:
\begin{align}\nonumber
  P(X) = P(g\cdot X) \quad \text{for all } g\in\grp \;.
\end{align} 
In probabilistic literature, it is often more convenient to obtain invariant joint distributions first. The joint distribution $P(X,Y)$ is invariant if and only if:
\begin{align}\nonumber
 (X,Y) = (g\cdot X, Y) \quad \text{for all } g\in\grp \;.
\end{align}
Then we can have the corresponding conditional distribution with the following proposition: \citep{kallenberg2017random,DBLP:journals/jmlr/Bloem-ReddyT20}:
\begin{proposition}\label{lemma:joint_symmetry}
Assume a group $\grp$ acting on $\gX$ and $\gY,$ and then $ P(Y|X)$ is $\grp$-invariant if and only if $(X,Y) \equdist (g\cdot X,Y)$ for all $g\in\grp$.
\end{proposition}

==> tabs/TUD_005.tex <==

\begin{table*}[h]
  \centering
  \caption{TUDatasets results, where each set samples 5\% of the  subgraphs based on the selected policy. Gray background indicates \ours-gnn outperforms DSS-GNN with the same selection policy.}
  \label{tab:TUDatasets}
\tiny
\resizebox{\textwidth}{!}{
  \begin{tabular}{lccccc|cc}
      \toprule
        \textsc{Method} &
        \textsc{MUTAG} &
        \textsc{PTC} &
        \textsc{PROTEINS} &
        \textsc{NCI1} &
        \textsc{NCI109} &
        \textsc{IMDB-B} &
        \textsc{IMDB-M}
        \\
      \midrule
        {\bf \textsc{DSS-GNN (ED)}} & 
        84.6$\pm$3.7 &
         61.0$\pm$7.6 &
         72.1$\pm$4.7 &
         82.0$\pm$2.0 &
         81.5$\pm$1.3 &
         75.5$\pm$4.3 &
         50.7$\pm$2.6\\
        {\bf \textsc{DSS-GNN (ND)}} & 
         85.8$\pm$5.2 &
          60.5$\pm$5.1 &
          71.2$\pm$3.9 &
         81.6$\pm$1.8 &
         81.6$\pm$1.2 &
         73.5$\pm$3.2 &
         51.3$\pm$2.5
         \\
        {\bf \textsc{DSS-GNN (EGO)}} & 
         85.9$\pm$5.3 &
          60.2$\pm$6.2 &
          72.5$\pm$4.4 &
         82.4$\pm$1.9 &
         81.9$\pm$1.0 &
         74.3$\pm$2.7 &
         50.6$\pm$3.1
         \\
        {\bf \textsc{DSS-GNN (EGO+)}} &
        85.9$\pm$3.4 &
          61.3$\pm$6.9 &
          72.3$\pm$3.6 &
         81.2$\pm$1.3 &
         81.9$\pm$1.6 &
         75.3$\pm$3.2 &
         51.5$\pm$3.0
         \\
        \midrule
        {\bf \textsc{ROSS-GNN (ED)}} & 
        \cellcolor{Gray}86.2$\pm$2.6 &
        \cellcolor{Gray}61.4$\pm$7.7 &
        \cellcolor{Gray}73.4$\pm$3.0 &
        \cellcolor{Gray}82.2$\pm$1.7 &
        \cellcolor{Gray}81.9$\pm$1.5 &
        74.3$\pm$2.3 &
        \cellcolor{Gray}51.8$\pm$2.1 \\
        {\bf \textsc{ROSS-GNN (ND)}} & 
        \cellcolor{Gray}86.7$\pm$5.3 &
        \cellcolor{Gray}61.3$\pm$4.2 &
        \cellcolor{Gray}72.5$\pm$3.1 &
        \cellcolor{Gray}82.6$\pm$1.4&
        \cellcolor{Gray}81.7$\pm$1.5 &
        \cellcolor{Gray}73.7$\pm$3.1 &
        \cellcolor{Gray}51.6$\pm$2.7
         \\
        {\bf \textsc{ROSS-GNN (EGO)}} & 
        \cellcolor{Gray}86.2$\pm$4.7 &
        \cellcolor{Gray}60.6$\pm$7,9 &
        \cellcolor{Gray}73.3$\pm$1.9 &
         82.1$\pm$1.7 &
        \cellcolor{Gray}82.2$\pm$1.3 &
        \cellcolor{Gray}75.0$\pm$1.6 &
        \cellcolor{Gray}51.8$\pm$2.6
         \\
        {\bf \textsc{ROSS-GNN (EGO+)}} &
        \cellcolor{Gray}86.2$\pm$5.3 &
        \cellcolor{Gray}61.5$\pm$6.4 &
        \cellcolor{Gray}72.9$\pm$4.6 &
        \cellcolor{Gray}82.8$\pm$1.4 &
        \cellcolor{Gray}82.5$\pm$1.1 &
         74.8$\pm$3.2 &
        \cellcolor{Gray}51.7$\pm$2.9
         \\
        
      \bottomrule
    \end{tabular}
    }
\end{table*}

==> tabs/product_recom.tex <==
\begin{table*}[h]
    
    \centering
    \caption{Product recommendation results on the Amazon dataset with different categories}\label{tab:product}


    \resizebox{\linewidth}{!}{
    \begin{tabular}{l | lllllllllll}
        \toprule
        &  
        \textbf{\quad Toys} &
         \textbf{\quad Gear} &
        \textbf{\quad Carseats} &
        \textbf{\quad Bath} &
         \textbf{\quad Health} &
         \textbf{\quad Diaper} &
         \textbf{\quad Bedding} &
         \textbf{\quad Feeding} &
         \textbf{\quad Apparel} &
        \textbf{\quad Media}
        \\
        \midrule       
        

         \multirow{1}{*}{\bf \textsc{Random}}  & 
         \quad0.083 &
         \quad0.077 &
         \quad0.066 &
         \quad0.076 &
         \quad0.076 &
         \quad0.084 &
         \quad0.079 &
         \quad0.093 &
         \quad0.090 &
         \quad0.094
         \\
        
        
                \midrule

         \multirow{1}{*}{\bf \textsc{DeepSet}}  & 
         0.421$\pm$0.005 &
         0.379$\pm$0.005&
         \textbf{0.205}$\pm$\textbf{0.008} &
         0.418$\pm$0.007 &
         0.452$\pm$0.001&
         0.451$\pm$0.003&
         0.481$\pm$0.002 &
         0.428$\pm$0.002 &
         0.508$\pm$0.004 &
         0.426$\pm$0.004
         \\
        
        
                \midrule

         \multirow{1}{*}{\bf \textsc{EquiVSet}}  & 
         0.684$\pm$0.004 &
         0.725$\pm$0.011 &
         0.200$\pm$0.019 &
         0.764$\pm$0.020 &
         0.705$\pm$0.009 &
         0.828$\pm$0.007 &
         0.762$\pm$0.005 &
         0.819$\pm$0.009 &
         0.764$\pm$0.005 &
         0.554$\pm$0.005
         \\
        
        
                \midrule

        \multirow{1}{*}{\bf \textsc{ROSS}}  & 
         \textbf{0.769}$\pm$\textbf{0.005} &
         \textbf{0.808}$\pm$\textbf{0.012} &
         0.202$\pm$0.014 &
         \textbf{0.862}$\pm$\textbf{0.005} &
         \textbf{0.812}$\pm$\textbf{0.005} &
         \textbf{0.880}$\pm$\textbf{0.007} &
         \textbf{0.857}$\pm$\textbf{0.010} &
         \textbf{0.885}$\pm$\textbf{0.005} &
         \textbf{0.837}$\pm$\textbf{0.003} &
         \textbf{0.620}$\pm$\textbf{0.023}
         \\
               
        
        \bottomrule

    \end{tabular}
    }
\end{table*}
